Rigid Body Path Planning using Mixed-Integer Linear Programming

Navigating rigid body objects through crowded environments can be challenging, especially when narrow passages are presented. Existing sampling-based planners and optimization-based methods like mixed integer linear programming (MILP) formulations, suffer from limited scalability with respect to either the size of the workspace or the number of obstacles. In order to address the scalability issue, we propose a three-stage algorithm that first generates a graph of convex polytopes in the workspace free of collision, then poses a large set of small MILPs to generate viable paths between polytopes, and finally queries a pair of start and end configurations for a feasible path online. The graph of convex polytopes serves as a decomposition of the free workspace and the number of decision variables in each MILP is limited by restricting the subproblem within two or three free polytopes rather than the entire free region. Our simulation results demonstrate shorter online computation time compared to baseline methods and scales better with the size of the environment and tunnel width than sampling-based planners in both 2D and 3D environments.

==> RAL-final/B-response.tex <==
% \documentclass[journal, onecolumn, 12pt]{IEEEtran}
% \usepackage{hyperref}
% \usepackage{color}
% \usepackage{soul}
% \usepackage{amsmath}
% \usepackage{cleveref}
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[font=footnotesize]{subcaption}
% \newtheorem{theorem}{Theorem}
% \newtheorem{proof}{Proof}

% \usepackage{enumitem}
% \setlist[enumerate,1]{itemsep=1em, parsep=0em}

% \newcommand{\mingxin}[1]{\textcolor{blue}{[MX: #1]}}
% % \newcommand{\finished}[1]{\textcolor{green}{#1}}

% \title{Statement of Changes}
% \begin{document}
% \maketitle

\begin{center}
    \LARGE{Statement of Changes}
    \vspace{1em}
\end{center}

The authors thank all RA-L reviewers and the editor of the IEEE Robotics and Automation Letter (RA-L) for their careful reviews. We hope the reviewers' concerns have now been adequately addressed. We appreciate your time and consideration throughout this review process and await our submission's final decision.

\section{Response to the editor}
Thank you for your summary. We have revised the paper as suggested:
\begin{enumerate}
    \item 
    \textbf{Advice: Contribution of this work and clarity.}
    
    \textbf{Response:} The focus of our work is navigating large objects through highly cluttered environments. Our method is an optimization-based algorithm which 
    1) operates directly within the workspace, mitigating the challenges associated with covering narrow tunnels in the free space, compared to configuration space-based approaches.
    2) improves online efficiency and guarantees the planned path to be collision-free without worrying about the resolution of collision checking. This is achieved by breaking down a large, complex optimization problem into a series of smaller MILP problems.
    \vspace{1em}\item 
    \textbf{Advice: lack of citation of prior work and more direct comparison to existing approaches.}
    
    \textbf{Response:} Thank you for the suggestion. We have included one more baseline of workspace-based connectivity oracle (WCO) in~\cref{sec:experiment}, which is a sampling-based method utilizing workspace information. We also added more discussion in~\cref{sec:related_work} with more citations of prior work.
    \vspace{1em}\item 
    \textbf{Advice: The reviewers note some limitations and the need for a more direct discussion of them.}
    
    \textbf{Response:} Thank you for the suggestion. We have included discussions of the limitations of our method in the response to the reviewers and in~\cref{subsec:limitation}. 
\end{enumerate}


\section{Response to reviewer-1 (350461)}
Thank you for your comments and suggestions. We have updated the paper and hope the following clarifications help to address your concerns.
\begin{enumerate}
    \item
    \textbf{Comment [limited scope]:} The targeted problem of geometric rigid-body motion planning is outdated and has limited applicability. Applying this method to more challenging problems, such as kinodynamic planning for drones or manipulators (as in the original GCS paper), would make it a more interesting contribution.

    \textbf{Response:} Thanks for your comment. While kinodynamic planning is indeed important, our work addresses critical challenges in navigating large objects through highly cluttered environments, which remains relevant in manipulation applications like assembly. Our algorithm improved online efficiency and guaranteed the planned path. to be collision-free. Furthermore, many intermediate computation results can be reusable.

    The online efficiency and result reusability of our algorithm make it particularly suitable for real-time applications and relatively fixed environments. This addresses a gap in current planning techniques for large object manipulation in complex environments.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [limited scope \& rotation in 3D]:} The proposed method imposes further constraints, such as allowing only translational movements on edges, which limits its scope. For 3D environments, the authors only allow robot translations. It is unclear if this restriction means the object cannot rotate at all or if it can rotate only within the region of the $V_d$ vertices. In any case this significantly reduces the applicability of the method, and makes the dimensionality of the problem significantly easier.

    \textbf{Response:} We appreciate the reviewer's comment on the limitations of our method in 3D scenarios. As stated, restricting the object to only translational movements in 3D simplifies the problem dimensionality and computational complexity. 
    This constraint only applies to 3D scenarios and was made deliberately for straight-forward collision-avoidance encoding in 3D. In 2D, both translational and rotational movements are allowed on the edges. However, approximating the reachable set when rotation is permitted in 3D is challenging.

    As for the applicability, our proposed method can still solve general problems in 3D environments. As illustrated in~\cref{fig:increase-env}, as more obstacles are added into the environment, our method will grow more convex polytope covers inside the free workspace, thus including more nodes into the planning graph $G_d$. A higher number of nodes in $G_d$ allows for more maneuvers in the planned path, enabling the solution of not only narrow-passage problems but also more general ones.
    
    We acknowledge our current 3D method excludes a subset of solutions where most convex covers are so narrow that the object cannot fully rotate within the free space, and only a small set of orientations are admissible. This limitation can be mitigated by extending our method to include 3D rotations in MILP using approximation techniques similar to those employed in 2D. We expect to further explore that in future work and we have included the discussion in~\cref{subsec:limitation}.

    In summary, while this design choice significantly reduces computational complexity, it still allows for the solution of general problems without severely impacting feasibility. We recognize this limitation and intend to address 3D rotations in future research.

    \begin{figure}[h]
    \vspace{6pt}
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/easy-soln.jpg}
        \caption{1 obstacle - solution}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/mid-soln.jpg}
        \caption{2 obstacles - solution}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/test.jpg}
        \caption{4 obstacles - solution}
    \end{subfigure} \\ \vspace{.5em}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/easy-decompose.jpg}
        \caption{1 obstacle - decomposition}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/mid-decompose.jpg}
        \caption{2 obstacles - decomposition}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[height=9em]{figs/demo-3d/testt.jpg}
        \caption{4 obstacles - decomposition}
    \end{subfigure}
    \caption{Three planning problems in 3D with an increasing number of obstacles. New obstacles are added to block the solution path from the previous problem. Our method solves more challenging problems incrementally by adding more polytope covers within the free space, allowing for more maneuvers in the solution paths. While the object is restricted to translational movements in 3D, this simplification enables straightforward collision-avoidance encoding while still permitting the solution of general problems. (a-c) show the solutions to the problem, and (d-f) show the convex polytope covers (blue) inside the free workspace, with a red dot indicating the center of each polytope.}
    \label{fig:increase-env}
\end{figure}
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [typo]: Syntactical and grammatical errors.}

    \textbf{Response:} We carefully reviewed the paper to improve the writing and resolve the errors. All changes are colored red in the resubmission.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [related work]:} I also find the related work a bit lacking. There are many methods in motion planning that use workspace information to guide search, especially for rigid motion planning. Examples includes [A-C], with some methods applying to more challenging problems such as kinodynamic planning.

    \textbf{Response:} Thanks for the suggestion. We have added the references you recommended and updated~\cref{sec:related_work} in the revision.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [writing]:} The pipeline description is not well-organized.
    % , frequently switching contexts between point robots and rigid bodies, making it difficult to follow. In general there are many references to later or previous part of the text making quite challenging to parse. Figure 2 is missing subscript labels (a, b, c), the fourth subfigure, are unclear. Specifically, it is unclear what the gray candidate edges represent or what "verified by MILP" means. Section IV.C is especially difficult to understand. The sentence "adjacent free configurations" is not clearly defined, and it was not very clear to me at what part of the previous introduced algorithm it refers to.

    \textbf{Response:} Thanks for the great suggestion. We have carefully revised and updated~\cref{sec:pipeline,,sec:non-point} without switching from point objects to rigid body objects. We also moved the discussion of constructing vertices $\mathcal V_d$ (previously detailed in Section IV.C) to the appendix and updated the discussion in~\cref{sec:dense_graph}.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [collision-free]:} There are concerns about the paths produced by the MILP being collision-free. The authors acknowledge that continuous collision checking constraints cannot be fully encoded in practice, leading them to split the path into 10 segments and check only end-points. This seems to allow for non-colliion free edges to be addes under a small resolution.

    \textbf{Response:} We appreciate your concern regarding collision-free paths. There may be a misunderstanding of our collision-checking methods. Our approach indeed employs a more rigorous method than endpoints checking alone. Our collision-free encoding works like this:
    \begin{enumerate}
        \item Discretization: we split the to-be-checked line segments into subdivisions.
        \item Collision checking for line segments: apart from checking the endpoints of subdivisions lying inside the convex polytopes (this is classified as 'less strict' encoding as shown in the left of~\cref{fig:collision-avoidance}), we also add one more constraint onto the endpoints. The additional constraint is to further enforce either a) the endpoints of the original line segment inside the same convex polytope or b) one endpoint of subdivisions lies in the intersection of two involved convex polytopes. This more strict encoding is shown through~\cref{thm:line} and in the middle figure of~\cref{fig:collision-avoidance}.
        \item Collision checking for reachable sets: Through two additional corollaries, we are able to show our encoding can be easily applied to certain polytopes, whose union forms our reachable set.
    \end{enumerate}
    Our implementation ensures collision-free trajectories without worrying about the resolution limits of the discretization. We also updated the caption of~\cref{fig:collision-avoidance} for better clarity.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [new baseline]:} compare against A PRM method that uses workspace information [A], or spends more time to build an efficient graph like SPARS [D] would be more appropriate.

    \textbf{Response:} Thank you for the suggestion. We've included a quantitative comparison against "Workspace-based connectivity oracle" (WCO [A]) in~\cref{tab:planning-general} and added a discussion comparing the efficiency in~\cref{subsec:compare-prm}. These comparisons demonstrate our algorithm's effectiveness in relation to sampling-based methods that leverage workspace information.
\end{enumerate}

\section{Response to reviewer-2 (352093)}
Thank you for your comments and suggestions. We have updated the paper and hope the following clarifications help to address your concerns.
\begin{enumerate}
    \item
    \textbf{Comment [complexity of problem]}: The significance of the original problem, however, could have been further emphasized with more citations, and the hardness of the problem (is it NP-hard?) could have been discussed.

    \textbf{Response:} We thank the reviewer for the suggestion. The general motion planning problem is shown to be PSPACE-hard w.r.t the number of degrees of freedom by [1], which implies NP-hardness. A more detailed discussion of the complexity over variants of planning problems can be found in [2], which also shows the PSPACE-hardness complexity w.r.t. the number of agents. However, when restricted to a single rigid-body object with fixed degrees of freedom, discussing complexity is challenging and not straightforward without specifying the parameter of interest.

    [1] J. H. Reif. Complexity of the mover's problem and generalizations. In Proceedings IEEE Symposium on Foundations of Computer Science, pages 421-427, 1979.
    
    [2] \href{https://lavalle.pl/planning/node303.html}{https://lavalle.pl/planning/node303.html}
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [minor typos]}

    \textbf{Response:} We carefully reviewed the paper to improve the writing and resolve the errors. All changes are colored red in the resubmission.
    % =========================================================================
    \vspace{1em}\item 
    \textbf{Comment [online query]}: The authors could have expanded a little on how path planning was performed on the final graph, had there been more space.

    \textbf{Response:} Thanks for the suggestion. We've added more details about the online query phase in~\cref{sec:inference} of the main manuscript.
\end{enumerate}

\section{Response to reviewer-3 (352095)}
Thank you for your comments and suggestions. We have updated the paper and hope the following clarifications help to address your concerns.
\begin{enumerate}
    \item 
    \textbf{Comment [fineness of discretization]:} The fineness of the discretization seems important: too fine and the problem becomes very large, too coarse and the solutions are not accurate. What is the complexity of the approach with respect to this discretization? Empirically, how coarse of discretization can we get away with before problems start to occur?
    
    \textbf{Response:} Thank you for this highlight. The fineness of discretization significantly impacts the size of the solution set. In our 2D experiments, we used the following discretization parameters (which are also included in the first paragraph of~\cref{sec:experiment}):
    \begin{itemize}
        \item The rotation $\theta$ is discretized as $N_\theta=12$ values, allowing rotation as small as $30^\circ$.
        \item The translation discretization on $\partial P_{ij}$ is $N_t=60$ points with equal intervals along the line ring.
        \item The discretization in collision avoidance is that each line segment to be checked is divided into $N_c=10$ equal parts.
    \end{itemize}
    The complexity of the discretization is: 
    \begin{itemize}
        \item The discretization of $\theta$ and translation will affect the construction of patches on $\partial P_{ij}$, thus affecting the total number of MILP to be solved. Not considering the grouping operation, the number of MILP will grow at the rate of $O(N_\theta \cdot N_t)$.
        \item Inside each MILP, the discretization parameter $N_c$ in collision avoidance only affects the number of constraints at the rate of $O(N_c)$ but has no effect on the number of variables. The discretization of $\theta$ and translation will affect the number of variables at the rate of $O(N_\theta+N_t)$ without affecting the number of constraints.
    \end{itemize}
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [key assumption]:} The authors assume that "the line segments extending from [an object's] geometric center to each vertex are entirely contained within the boundaries of the object." How restrictive is this assumption? This assumption does not seem to hold for the example "L" shape. Does this mean that the planner is essentially considering the convex hull of the object shape?

    \textbf{Response:} Thank you for catching this. The previous description of the assumption is indeed not accurate, and we'd like to revise and clarify it as follows:
    \begin{enumerate}
        \item Assumption: the object's geometric center be properly selected to avoid falling out of the region, instead of enforcing all center-to-vertex lines to be within the object. We've modified the statement at the beginning of~\cref{sec:non-point}.
        \item Overapproximation as convex hull: No, our method is not planning for the convex hull of the original object. Our method plans for the area enclosed by a) the object edges and b) all the line segments connecting the geometric center with the vertices.
        \item Take the "L" shape as an example:\begin{itemize}
            \item The origin of the object is selected as the center of its longer branch in our experiments. In this case, as shown in~\cref{fig:2d-peg-in-hole}, we are computing the union of the "L" and a triangle (convex hull of the corner of "L").
            \item The origin of the object can also be selected as the corner of "L", and our method will be planning for the exact geometry of "L".
        \end{itemize}
    \end{enumerate}
    Our method does not use the convex hull but may consider a slightly larger area than the object itself, which enables better encoding of the collision-avoidance constraint during movement.
    We've updated the paper to clarify this methodology and its implications.
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [convex hull]:} What happens with a very large irregularly shaped object that can barely squeeze around obstacles? I.e., the convex hull would not fit but the object does fit? Can the approach handle this sort of thing? If so, it would be nice to see an example. If not, it would be nice to understand why.

    \textbf{Response:} Thank you for the question. Continuing the above discussion, we've included one example~\cref{fig:convex_hull} in 2D demonstrating that our method is not computing for the convex hull and is able to squeeze in some challenging environments. The agent is of "V" shape and its convex hull cannot squeeze into this environment.
    \begin{figure}[h]
        \centering
        \includegraphics[width=0.5\linewidth]{figs//main-env_vis/chull-2D.pdf}
        \caption{A large non-convex V-shaped object squeezes around the obstacles (Also serves as \cref{fig:enter-label} in the main manuscript). Our method is able to find a solution inside the challenging environment.}
        \label{fig:convex_hull}
    \end{figure}
    % =========================================================================
    \vspace{1em}\item
    \textbf{Comment [rotation in 3D]:} The reviewer is a bit confused by the statement "In 3D, only translation is allowed." If the proposed approach can't generate rotations in 3D, it doesn't seem very useful. I can't quite tell if there is a rotation in Figure 5.h, but it looks like there might be one. So perhaps I am misunderstanding this statement? An example with clear 3D rotations, perhaps with a small video, would make the paper much more convincing.

    \textbf{Response:} Thank you for raising the question. In~\cref{subsubsec:reachable}, we stated that "in 3D, only translation is allowed". This is indeed an abbreviation of that: the robot can only translate inside the MILP problem, and rotation is only allowed inside each $V_d$ vertices. We have updated the paragraph in~\cref{subsubsec:reachable} and also included a supplementary video to demonstrate 3D rotation for your reference.
    % =========================================================================
    \vspace{1em}\item 
    \textbf{Comment [comparison against GCS]:} The authors mention that compared with GCS in configuration space, the proposed method is less optimal but tends to be faster. Does it also have a smaller set of solutions? Are there problem instances for which GCS has a solution but the proposed approach does not? It seems like there should be, as the proposed approach is baking in extra assumptions to allow for greater computational efficiency.

    \textbf{Response:} Thanks for the insightful question. The comparison between our method and GCS is nuanced. The size of the solution set largely depends on hyperparameter choices. 
    
    For our method in 2D, our solution set will expand if we a) add more convex covers in the workspace, b) increase the waypoint number inside MILP $N$ or c) increase the fineness of discretization on the surface $\partial P_{ij}$. 
    Moreover, as we discussed before in comment 2), if all the vertice-to-center line segments lie inside the planned object, our method plans for the exact geometry of the object and can eliminate the missing set of solutions eventually. 
    
    In 3D, our current method solves increasingly challenging problems by adding more convex polytopes into the free workspace, as illustrated in~\cref{fig:increase-env}. This results in more nodes being included in the planning graph $G_d$, allowing for more maneuvers in the planned path and enabling the solution of both narrow-passage and more general problems.
    We acknowledge that our current 3D method excludes a subset of solutions where most convex covers are so narrow that the object cannot fully rotate within the free space, and only a small set of orientations are admissible. 

    GCS also faces completeness challenges. The missing set of solutions comes from failing to cover some free regions in the free configuration space. As free regions in the configuration space are highly non-convex, diminishing missing solutions is more challenging. Requires manual seeding or more advanced seeding techniques and a much longer optimization time as the number of convex sets increases.

    There are clear tradeoffs between the two approaches. Our method is potentially faster but may miss some solutions in complex scenarios. GCS can be more complete at the cost of intensive computation, as the number of convex sets increases.

    For future work, we aim to extend our 3D MILP to include rotation, which will expand the solution set. We also plan to develop adaptive parameter tuning to balance completeness and efficiency.
    
    
    % One key bottleneck for GCS to perform well is a properly generated graph of convex sets, which relies on finding appropriate seeds to generate the convex regions inside the configuration space. If there are too many overlaps between the convex sets, it will requires a larger amount of sets to cover the free space and the optimization problem will be much larger and exponentially slower. If the number of convex sets is too small, the convex sets may be disjoint and one will fail to find a solution. We expect that via manual seeding or more advanced sampling methods, GCS will be able to overcome the challenge and be more efficient.

    % For our method, the challenge is mitigated as the cover of convex set is generated in workspace.
    
\end{enumerate}

\section{List of Changes}
\begin{enumerate}
    \item Corrected the assumptions at the beginning of~\cref{sec:non-point}.
    \item Added one baseline method of Workspace-based Connectivity Oracle (WCO) in~\cref{sec:experiment}, mainly in~\cref{tab:planning-general,,subsec:compare-prm}.
    \item Added relevant works and updated discussions in~\cref{sec:related_work}.
    \item Added a supplementary video to demonstrate 3D rotation of the solution we found.
    \item Moved the previous discussion about constructing vertices $\mathcal V_d$ in Section IV.C to Appendix A. And updated related discussion in~\cref{sec:dense_graph}.
    \item Reorganized~\cref{subsec:limitation} and added more discussion.
    \item Changed the example figure in~\cref{fig:enter-label}.
    \item Corrected the typos and improved writing.
\end{enumerate}

% \end{document}
